Design-Based Inference with AI Predictions

We extend and refine prediction-powered inference for linear functionals of a regression, including treatment effects and average derivatives, when outcome labels are scarce. The study design supplies a known Riesz representer, whose weights give an exact correction for prediction errors. Under independent labeled and target sampling, the resulting estimator is unbiased for every admissible fixed predictor. We fit AI-assisted predictors to minimize the empirical variance of weighted residuals. We establish asymptotic variance optimality within a possibly misspecified prediction class when the labeled sample is asymptotically smaller than the target sample. Linear prediction classes yield transformed least squares. Our conditions for valid cross-fitted inference allow a misspecified limit without imposing a regression convergence rate. We also develop full-variance optimization through direct fitting and stacking at general sample-size ratios. Resampling the OpenResearch Unconditional Income Study illustrates these precision gains. With 10% of each arm labeled, stacking learners that combine few-shot predictions, covariates, and AI-generated features reduces variance relative to labeled-only estimation by 15.3% to 45.6% across fourteen outcomes. Its 95% intervals contain the full-cohort benchmark in 94.7% of replicates on average.

==> tab_full_body.tex <==
\multicolumn{9}{l}{\textbf{Expenditure}} \\
\multicolumn{9}{l}{\quad Total spending} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 329.5 & $-$0.2 & 207 & 0.958 & 0.958 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.215 & 0.215 & 339.9 & $+$10 & 183 & 0.991 & 0.991 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.157 & 0.157 & 341.1 & $+$11 & 190 & 0.963 & 0.964 \\
\qquad M1 & stacked & -- & 0.209 & 338.3 & $+$8.6 & 184 & -- & 0.961 \\
\qquad M2 & stacked & -- & 0.229 & 334.2 & $+$4.4 & 182 & -- & 0.954 \\
\qquad M3 & stacked & -- & 0.255 & 342.8 & $+$14 & 182 & -- & 0.958 \\
\qquad M4 & stacked & -- & \textbf{0.367} & 320.9 & $-$8.2 & 168 & -- & 0.951 \\
\multicolumn{9}{l}{\quad Food} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 60.87 & $-$0.2 & 59.5 & 0.955 & 0.955 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.284 & 0.284 & 51.68 & $-$9.4 & 50.4 & 0.990 & 0.990 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.174 & 0.170 & 49.34 & $-$12 & 54.2 & 0.953 & 0.955 \\
\qquad M1 & stacked & -- & 0.283 & 53.20 & $-$7.9 & 50.4 & -- & 0.958 \\
\qquad M2 & stacked & -- & \textbf{0.345} & 56.92 & $-$4.2 & 48.2 & -- & 0.955 \\
\qquad M3 & stacked & -- & 0.343 & 57.89 & $-$3.2 & 48.3 & -- & 0.956 \\
\qquad M4 & stacked & -- & 0.328 & 55.74 & $-$5.4 & 48.9 & -- & 0.954 \\
\multicolumn{9}{l}{\quad Rent} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 64.00 & $-$1.5 & 78.8 & 0.951 & 0.951 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.262 & 0.262 & 46.33 & $-$19 & 67.7 & 0.945 & 0.945 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.271 & 0.270 & 46.65 & $-$19 & 67.3 & 0.944 & 0.945 \\
\qquad M1 & stacked & -- & 0.251 & 49.05 & $-$16 & 68.2 & -- & 0.941 \\
\qquad M2 & stacked & -- & 0.251 & 49.69 & $-$16 & 68.2 & -- & 0.941 \\
\qquad M3 & stacked & -- & \textbf{0.313} & 53.12 & $-$12 & 65.3 & -- & 0.943 \\
\qquad M4 & stacked & -- & 0.311 & 51.25 & $-$14 & 65.4 & -- & 0.940 \\
\multicolumn{9}{l}{\quad Car} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 29.43 & $+$1.4 & 44.3 & 0.954 & 0.954 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.161 & 0.161 & 39.62 & $+$12 & 40.5 & 0.968 & 0.968 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.114 & 0.108 & 40.90 & $+$13 & 41.8 & 0.955 & 0.957 \\
\qquad M1 & stacked & -- & 0.177 & 36.00 & $+$8 & 40.2 & -- & 0.954 \\
\qquad M2 & stacked & -- & 0.178 & 36.10 & $+$8.1 & 40.1 & -- & 0.949 \\
\qquad M3 & stacked & -- & 0.179 & 36.24 & $+$8.2 & 39.8 & -- & 0.951 \\
\qquad M4 & stacked & -- & \textbf{0.187} & 34.61 & $+$6.6 & 39.6 & -- & 0.953 \\
\addlinespace
\multicolumn{9}{l}{\textbf{Employment \& income}} \\
\multicolumn{9}{l}{\quad Work hours} \\
\qquad Floor & labeled-only DiM & 0 & 0 & $-$1.706 & $+$0.078 & 2.41 & 0.958 & 0.958 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.157 & 0.157 & $-$1.607 & $+$0.18 & 2.21 & 0.968 & 0.968 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.118 & 0.118 & $-$1.587 & $+$0.2 & 2.26 & 0.959 & 0.959 \\
\qquad M1 & stacked & -- & 0.177 & $-$1.623 & $+$0.16 & 2.18 & -- & 0.960 \\
\qquad M2 & stacked & -- & 0.183 & $-$1.540 & $+$0.24 & 2.18 & -- & 0.959 \\
\qquad M3 & stacked & -- & \textbf{0.213} & $-$1.615 & $+$0.17 & 2.11 & -- & 0.962 \\
\qquad M4 & stacked & -- & 0.212 & $-$1.627 & $+$0.15 & 2.11 & -- & 0.959 \\
\multicolumn{9}{l}{\quad Employed} \\
\qquad Floor & labeled-only DiM & 0 & 0 & $-$0.02982 & $+$0.0000 & 0.0458 & 0.960 & 0.960 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.189 & 0.189 & $-$0.03011 & $-$0.00027 & 0.0412 & 0.965 & 0.965 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.187 & 0.189 & $-$0.02978 & $+$0.0001 & 0.0412 & 0.960 & 0.962 \\
\qquad M1 & stacked & -- & 0.184 & $-$0.02982 & $+$0.0000 & 0.0413 & -- & 0.960 \\
\qquad M2 & stacked & -- & 0.185 & $-$0.03046 & $-$0.00062 & 0.0413 & -- & 0.959 \\
\qquad M3 & stacked & -- & \textbf{0.241} & $-$0.02671 & $+$0.0027 & 0.0405 & -- & 0.963 \\
\qquad M4 & stacked & -- & 0.235 & $-$0.02550 & $+$0.0039 & 0.0406 & -- & 0.961 \\
\multicolumn{9}{l}{\quad Couple hours} \\
\qquad Floor & labeled-only DiM & 0 & 0 & $-$2.426 & $+$0.017 & 3.17 & 0.956 & 0.956 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.220 & 0.220 & $-$2.275 & $+$0.17 & 2.80 & 0.962 & 0.962 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.202 & 0.202 & $-$2.278 & $+$0.17 & 2.83 & 0.955 & 0.960 \\
\qquad M1 & stacked & -- & 0.227 & $-$2.278 & $+$0.17 & 2.78 & -- & 0.957 \\
\qquad M2 & stacked & -- & 0.231 & $-$2.357 & $+$0.086 & 2.78 & -- & 0.957 \\
\qquad M3 & stacked & -- & 0.244 & $-$2.368 & $+$0.075 & 2.75 & -- & 0.956 \\
\qquad M4 & stacked & -- & \textbf{0.247} & $-$2.316 & $+$0.13 & 2.75 & -- & 0.955 \\
\multicolumn{9}{l}{\quad Labor index} \\
\qquad Floor & labeled-only DiM & 0 & 0 & $-$0.08198 & $+$0.0032 & 0.117 & 0.962 & 0.962 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.198 & 0.198 & $-$0.07963 & $+$0.0056 & 0.104 & 0.967 & 0.967 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.190 & 0.189 & $-$0.08050 & $+$0.0047 & 0.105 & 0.959 & 0.960 \\
\qquad M1 & stacked & -- & 0.199 & $-$0.07997 & $+$0.0053 & 0.104 & -- & 0.960 \\
\qquad M2 & stacked & -- & 0.197 & $-$0.07860 & $+$0.0066 & 0.105 & -- & 0.956 \\
\qquad M3 & stacked & -- & 0.242 & $-$0.08795 & $+$0.005 & 0.110 & -- & 0.952 \\
\qquad M4 & stacked & -- & \textbf{0.248} & $-$0.08840 & $+$0.0045 & 0.110 & -- & 0.954 \\
\multicolumn{9}{l}{\quad HH income} \\
\qquad Floor & labeled-only DiM & 0 & 0 & $-$4.811 & $+$0.0089 & 3.85 & 0.955 & 0.955 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.238 & 0.238 & $-$4.536 & $+$0.28 & 3.36 & 0.981 & 0.981 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.194 & 0.190 & $-$4.425 & $+$0.4 & 3.46 & 0.958 & 0.957 \\
\qquad M1 & stacked & -- & 0.233 & $-$4.523 & $+$0.3 & 3.37 & -- & 0.958 \\
\qquad M2 & stacked & -- & 0.307 & $-$4.902 & $-$0.082 & 3.20 & -- & 0.954 \\
\qquad M3 & stacked & -- & 0.320 & $-$4.937 & $-$0.12 & 3.17 & -- & 0.956 \\
\qquad M4 & stacked & -- & \textbf{0.325} & $-$4.810 & $+$0.01 & 3.16 & -- & 0.961 \\
\multicolumn{9}{l}{\quad Own income} \\
\qquad Floor & labeled-only DiM & 0 & 0 & $-$2.059 & $+$0.098 & 3.61 & 0.952 & 0.952 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.170 & 0.170 & $-$2.580 & $-$0.42 & 3.29 & 0.957 & 0.957 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.170 & 0.167 & $-$2.731 & $-$0.57 & 3.30 & 0.946 & 0.946 \\
\qquad M1 & stacked & -- & 0.168 & $-$2.549 & $-$0.39 & 3.30 & -- & 0.950 \\
\qquad M2 & stacked & -- & 0.185 & $-$2.550 & $-$0.39 & 3.26 & -- & 0.949 \\
\qquad M3 & stacked & -- & 0.187 & $-$2.512 & $-$0.36 & 3.08 & -- & 0.960 \\
\qquad M4 & stacked & -- & \textbf{0.193} & $-$2.507 & $-$0.36 & 3.06 & -- & 0.965 \\
\addlinespace
\multicolumn{9}{l}{\textbf{Financial health \& saving}} \\
\multicolumn{9}{l}{\quad HH saving} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 0.04532 & $+$0.0019 & 0.0379 & 0.957 & 0.957 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.320 & 0.320 & 0.04862 & $+$0.0052 & 0.0312 & 0.965 & 0.965 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.314 & 0.310 & 0.04860 & $+$0.0051 & 0.0314 & 0.959 & 0.960 \\
\qquad M1 & stacked & -- & 0.325 & 0.04805 & $+$0.0046 & 0.0311 & -- & 0.963 \\
\qquad M2 & stacked & -- & 0.331 & 0.04659 & $+$0.0031 & 0.0310 & -- & 0.957 \\
\qquad M3 & stacked & -- & 0.338 & 0.04498 & $+$0.0015 & 0.0308 & -- & 0.960 \\
\qquad M4 & stacked & -- & \textbf{0.366} & 0.04640 & $+$0.0029 & 0.0301 & -- & 0.964 \\
\multicolumn{9}{l}{\quad Own saving} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 0.04335 & $+$0.0014 & 0.0384 & 0.961 & 0.961 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.149 & 0.149 & 0.05336 & $+$0.011 & 0.0354 & 0.953 & 0.953 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.159 & 0.155 & 0.05246 & $+$0.01 & 0.0353 & 0.955 & 0.956 \\
\qquad M1 & stacked & -- & 0.188 & 0.05022 & $+$0.0082 & 0.0346 & -- & 0.961 \\
\qquad M2 & stacked & -- & \textbf{0.268} & 0.04978 & $+$0.0078 & 0.0328 & -- & 0.960 \\
\qquad M3 & stacked & -- & 0.267 & 0.04894 & $+$0.007 & 0.0329 & -- & 0.962 \\
\qquad M4 & stacked & -- & 0.258 & 0.04627 & $+$0.0043 & 0.0331 & -- & 0.968 \\
\multicolumn{9}{l}{\quad FH index} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 0.7066 & $-$0.00023 & 0.861 & 0.957 & 0.957 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.442 & 0.442 & 0.6001 & $-$0.11 & 0.644 & 0.983 & 0.983 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.437 & 0.436 & 0.6167 & $-$0.09 & 0.647 & 0.958 & 0.960 \\
\qquad M1 & stacked & -- & 0.434 & 0.5967 & $-$0.11 & 0.648 & -- & 0.956 \\
\qquad M2 & stacked & -- & 0.438 & 0.6078 & $-$0.099 & 0.646 & -- & 0.958 \\
\qquad M3 & stacked & -- & 0.463 & 0.6023 & $-$0.1 & 0.631 & -- & 0.957 \\
\qquad M4 & stacked & -- & \textbf{0.464} & 0.6061 & $-$0.1 & 0.631 & -- & 0.958 \\
\multicolumn{9}{l}{\quad FH self-rating} \\
\qquad Floor & labeled-only DiM & 0 & 0 & 0.09241 & $-$0.0026 & 0.118 & 0.960 & 0.960 \\
\qquad Fixed PPI & $f = p$, nothing fitted & 0.285 & 0.285 & 0.08954 & $-$0.0054 & 0.0995 & 0.969 & 0.969 \\
\qquad PPI++ & $f = \hat\lambda p$ & 0.275 & 0.275 & 0.09004 & $-$0.0049 & 0.100 & 0.960 & 0.958 \\
\qquad M1 & stacked & -- & 0.311 & 0.09074 & $-$0.0042 & 0.0977 & -- & 0.960 \\
\qquad M2 & stacked & -- & 0.410 & 0.08435 & $-$0.011 & 0.0905 & -- & 0.957 \\
\qquad M3 & stacked & -- & 0.419 & 0.08284 & $-$0.012 & 0.0897 & -- & 0.955 \\
\qquad M4 & stacked & -- & \textbf{0.420} & 0.08277 & $-$0.012 & 0.0897 & -- & 0.955 \\

